Network Representation Learning: Consolidation and Renewed Bearing

Graphs are a natural abstraction for many problems where nodes represent entities and edges represent a relationship across entities. An important area of research that has emerged over the last decade is the use of graphs as a vehicle for non-linear dimensionality reduction in a manner akin to previous efforts based on manifold learning with uses for downstream database processing, machine learning and visualization. In this systematic yet comprehensive experimental survey, we benchmark several popular network representation learning methods operating on two key tasks: link prediction and node classification. We examine the performance of 12 unsupervised embedding methods on 15 datasets. To the best of our knowledge, the scale of our study -- both in terms of the number of methods and number of datasets -- is the largest to date. Our results reveal several key insights about work-to-date in this space. First, we find that certain baseline methods (task-specific heuristics, as well as classic manifold methods) that have often been dismissed or are not considered by previous efforts can compete on certain types of datasets if they are tuned appropriately. Second, we find that recent methods based on matrix factorization offer a small but relatively consistent advantage over alternative methods (e.g., random-walk based methods) from a qualitative standpoint. Specifically, we find that MNMF, a community preserving embedding method, is the most competitive method for the link prediction task. While NetMF is the most competitive baseline for node classification. Third, no single method completely outperforms other embedding methods on both node classification and link prediction tasks. We also present several drill-down analysis that reveals settings under which certain algorithms perform well (e.g., the role of neighborhood context on performance) -- guiding the end-user.

==> backup.tex <==

\section{Tasks}
In order to evaluate the quality of the embeddings generated by the models described in \label{section: models}, we conducted experiments on two tasks - node classification and link prediction.

\subsection{Node Classification}
\subsubsection{Definition}
In complex networks, a subset of the nodes may contain labels which represent certain characteristics of the node. For example, nodes (users) in a social network may contain labels that denote geographic information, community membership or topics of interest. Node classification is the task of learning a classifier which, given the embedding of the node, can accurately predict the assigned label for that node. 

\subsubsection{Metrics}
%% TODO: Consider optimizing for space here by substituting for Precision and Recall
The following metrics were used to evaluate the performance of the trained classifier:

\textbf{F1-score}: Harmonic mean of the precision and recall. It is defined by: 
$$ 
F1 = \frac{2 \times Precision \times Recall}{ Precision + Recall }
$$
where,
$$ Precision = \frac{TP}{TP+FP} $$ $$ Recall = \frac{TP}{TP + FN} $$

\textit{Micro-F1}: Calculates the F1 score by counting the total $TP, FN$ and $FP$ across all classes.

$$
Precision = \frac{\sum_{i=0}^{k}TP_i}{\sum_{i=0}^{k}TP_i + \sum_{i=0}^{k}FP_i}
$$

Recall is derived similarly.

\textit{Macro-F1}: Calculates the un-weighted mean of the F1-score for the individual classes. 
$$ 
Macro-F1 = \sum_{i=0}^{k} \frac{2 \times Precision \times Recall}{ Precision + Recall }
$$

\textbf{Accuracy}: Calculates the number of correct predictions across all the predictions made by the model.

$$
Accuracy = \frac{TP+FN}{TP+FP+TN+FN}
$$

Here $TP$, $TN$, $FP$ and $FN$ denote \textit{True Positive, True Negative, False Positive} and \textit{False Negative} respectively. $k$ denotes the number of classes.

%----------------


\begin{table}[]
\begin{tabular}{llll}
\hline
\textbf{Baseline\textbackslash{}Paper} & DeepWalk & Node2vec & GraRep \\ \hline
DeepWalk & \color{red}{27.3} & \color{red}{21.1} & 26.85 \\
Node2vec & N/A & 25.8 & N/A \\
GraRep & N/A & Not Compared & \color{blue}{28.35} \\ \hline
Spectral Clustering & \color{blue}{28.31} & 4.05 & 24.83 \\
\hline
\end{tabular}
\caption{The reported Macro-F1 of baselines (rows) mentioned in the research papers (columns) for the task of multilabel node classification on BlogCatalog dataset with 50\% training data. N/A refers to not applicable and refers to cases where the method was proposed before the baseline was proposed.}
\label{comparison}
\end{table}

%----------------

==> methods_new.tex <==
\label{network_methods}
In this section, we provide a summary of the different network embedding methods considered in our study.Herein, for each models along with their description, we also report the considered hyper-parameter search space and also any additional experimental setting or insights we considered or observed during our evaluation. 


\begin{enumerate}

\item \textbf{Laplacian Eigemaps \cite{belkin2003laplacian}}: For a given graph, $G$, Laplacian Eigemaps provides a $d$-dimensional embedding, $U$, using the smallest $d$ eigenvectors of Laplacian matrix $L = D-A$.  This  Eigen Value Decomposition problem solves the following objective.
\begin{equation*}
\begin{aligned}& \underset{U}{\text{minimize}}& & trace(U^TLU) \\
& \text{subject to}& & U^TDU = I
\end{aligned}
\end{equation*}
The obtained orthonormal embeddings, $U$, can be seen as preserving the first order local information by making nodes connected in the graph lie closer in the embedding space under the L2 distance i.e $ \Sigma_{i,j} ||U^{(i)}-U^{(j)}||^2A_{ij}$, $ \forall (i,j) \in |V|*|V|$. Also, It has been shown that the problem of minimizing graph cuts can be approximately reduced to solving the Laplacian eigen maps and this made it a popular choice in the previous decade for clustering nodes.

\textbf{Comments}: We search for following  hyper parameters: Embedding dimension $\in$ [64, 128, 256]. On datasets with $> $1M nodes, we have reported results only for 64 dimensional space as it did not scale for 128 and 256 dimensions on a modern machine.


\item \textbf{DeepWalk \cite{perozzi2014deepwalk}}: 
DeepWalk is a random walk based model that provides embeddings that preserve a higher order neighborhood similarity corresponding to a pre-defined neighborhood context, $w$. Given a set of random walks with a certain length, DeepWalk learns embeddings for each node such that, the dot product distance between any node and it's neighbor that is reachable within $w$ steps of a random walk from the node in either direction is maximized. DeepWalk learns such embeddings by adapting the popular Skip-gram objective (Eqn: ) which was proposed initially to learn word embeddings in natural languages. In DeepWalk, an analogous artificial language was created for each graph where random walks formed sentences with the vocabulary defined by node identifiers. For every sub-sequence of context window, $w$ in a random walk with node $u$ anchored at the center, the following objective is solved to obtain the node embeddings, $\Phi(u)$. Since the conventional one-hot prediction of node ids will grow at $O(|V|)$, candidate sampling techniques such as Negative Sampling or Hierarchical Softmax can be used to scale for large graphs. 

\begin{equation}
minimize_{\Phi} \; - \log Pr(\{u_{i-w},\cdots, u_{i+w} \} \backslash  u_i \; | \; \Phi(u_i))
\end{equation}

\textbf{Comments}: We search for following hyper-parameters: Walk length $\in$ [5, 20, 40], Number of walks $\in$ [20, 40, 80], Window size ($w$)  $\in$ [ 2, 4, 10], Embedding dimension $\in$ [64, 128, 256]. To scale to large graphs, Hierarchical Softmax is used as the default strategy. In the case of directed graphs, we observed lower performance in node classification and link prediction task. In order to have a fair comparison with other methods, we treat directed graphs as undirected for DeepWalk.

\item \textbf{Node2Vec \cite{grover2016node2vec}}: Node2Vec builds upon DeepWalk, where the model feeds in a predefined biased random walk instead of the standard diffusion random walks to the Skip-gram model. The biased random walks are generated by trading off between the Breadth-first traversal and Depth-first traversal with two hyper parameters, $p, q$. The values for $p,q$ are tuned to maximize the end task's performance on a validation set. 

\textbf{Comments}: We search for following  hyper parameters: Walk length $\in$ [10, 20, 40], Number of walks = 80, Window Size = 10, $p$ and $q$ $\in$ [0.25, 1, 2, 4], Embedding dimension $\in$ [64, 128, 256]. By default, Node2Vec resorts to negative sampling based implementation.  Similar to DeepWalk, we observed lower performance on directed graphs on the classification task and hence we treated directed graphs as undirected for Node2Vec.


\item \textbf{GraRep \cite{cao2015grarep}}: 


GraRep is a matrix factorization based network embedding method which captures the global structural information of the graph while learning node embeddings. The authors observe that the existing Skipgram based models project all the $k$-step relational information into a common subspace and then, argue the importance of preserving different $k$-step relational information in separate subspaces. The loss function to preserve the $k$-step relationship between node $w$ and $c$ is proposed as: 

\begin{equation}
\begin{aligned}
L_k(u, v) = & A_{u, v}^{k}\cdot\log{\sigma(\Phi(u) \cdot \Phi(v))} \\ + & \frac{\lambda}{|V|}\sum\limits_{v' \in V, v' \ne v}{A_{u, v'}^k \cdot \log{\sigma(-\Phi(u)\cdot\Phi(v'))}}
\end{aligned}
\end{equation}


\vspace{-0.5em}

where $v'$ refers to the negative node at $k$-th step for node $u$ and $\lambda$ refers to the number of negative samples, 
The above loss function in closed form results in log-transformed, probabilistic adjacency matrix which is factorized with SVD for generating each $k$-step representation. The final node representation or embeddings is generated by concatenation of all the $k$-step representations.

\textbf{Comments}: We search for following  hyperparameters: $k$ from 1 to 6, Embedding dimension = [64, 128, 256]. On the datasets with $>$2M edges, due to scalability issue, we searched for $k$ from 1 to 2 and Embedding dimension = [64, 128].


\item \textbf{NetMF \cite{qiu2018network}}: NetMF is a matrix factorization based network embedding method. NetMF presents theoretical proofs for their claim that skip-gram models with negative sampling are implicitly approximating and factorizing appropriate matrices constructed with the help of graph Laplacians. The objective matrix based for NetMF on small context window T is given by
\begin{equation}
    M = \frac{vol(G)}{\lambda*T} \Big(\sum_{r=1}^{T} P^r \Big)D^{-1}
\end{equation}
NetMF factorizes the above closed form DeepWalk matrix with SVD in order to generate node embedding and provides two algorithms for small context window and large context window.

\textbf{Comments}: We search for following  hyperparameters: $T$ = [1, 10], Negative samples $\lambda$ = [1, 2, 3], Rank $H$ for large context window  = [128, 256, 512], Embedding dimension = [64, 128, 256].


\item \textbf{M-NMF \cite{wang2017community}}: M-NMF is a matrix factorization based network embedding method which generates node embeddings that preserves the microscopic information in form of first-order and second-order proximities among nodes and the generated embeddings also preserves mesoscopic information in form of community structure. The objective function for M-NMF is given as 
\begin{equation} 
\begin{aligned}
 O = \min_{ U,V C, H \geq 0} & {\lVert S-VU^{T} \rVert}^2 + \alpha * {\lVert H-UC^{T} \rVert}^2_F \\ & - \beta {tr}(H^TBH) + \zeta {\lVert HH^T-I \rVert}^2_F
\end{aligned}
\end{equation}
where $H$ is the binary community membership matrix, $C$ is the latent representations of communities and $B$ is the modularity matrix obtained from the adjacency matrix $A$. Overall, M-NMF discovers communities through modularity constraints. The node embeddings generated with the help of microscopic information and community embeddings are then, jointly optimized by assuming consensus relationship between both node and community embeddings.

\textbf{Comments}: We search for following  hyperparameters: $\alpha$ = [0.1, 1.0, 10.0], $\beta$ = [0.1, 1.0, 10.0], Embedding dimension = [64, 128, 256].

\item \textbf{HOPE \cite{ou2016asymmetric}}: HOPE is a matrix factorization based network embedding method which generates node embeddings that preserve asymmetric transitivity of nodes in directed graphs. If there exists a directed edge from node $u$ to $w$ and $w$ to $v$, then  -- due to asymmetric transitivity property -- an edge from $u$ to $v$ is more likely to form than edge from $v$ to $u$. The objective function of HOPE is given as follows
\begin{equation}
    min \;  \| S - U^s(U^t)^T \|^2_2
\end{equation}
where $U^s$ and $(U^t)$ are the source and target embeddings. In order to preserve asymmetric transitivity of nodes, the proximity matrix $S$ is constructed using a similarity metric which respects the directionality of edges. The node embeddings are generated by factorizing the proximity matrix with generalized SVD \cite{paige1981towards}.

\textbf{Comments}: We search for following  hyperparameters: The decay parameter $\beta$ = 0.5/(Spectral Radius of Graph). Embedding dimension = [64, 128, 256].


\item \textbf{LINE \cite{tang2015line}}: LINE is an optimization-based network embedding method which optimizes an objective function that preserves both first and second order proximity among nodes in the embedding space. The objective function for first-order proximity is given as
\begin{equation}
    O_1 = -\sum_{(u,v) \in E} A_{u,v} \; log \; \sigma(\Phi(u). \Phi(v))
\end{equation}
while the objective function to preserve the second order proximity is given as
\begin{equation}
    O_2 = -\sum_{(u,v) \in E} A_{u,v}  \; log \; \frac{exp(\Phi(u). \psi(v))}{\sum_{v' \in V, \substack{v' \ne v}} exp(\Phi(u). \psi(v'))}
\end{equation}

where $u'$ represents the node embedding of node $u$ and $\hat{v}, \hat{w}$ represents the context embedding of nodes $v$ and $w$ respectively. The first order proximity corresponds to local proximity between nodes based on the presence of edges in the graph while the second order proximity corresponds to global proximity between nodes based on shared neighborhoods of those nodes in the graph. Since the objective function is expensive to compute for large graphs, it is approximated by negative sampling \cite{MikolovWord2vec}.

\textbf{Comments}: We search for following  hyperparameters: Number of samples = 10 billion, Embedding dimension $\in$ [64, 128, 256]. In the case of directed graphs, as suggested by the authors of LINE, we evaluate only second-order proximity.


\item \textbf{Verse \cite{tsitsulin2018verse}}: Verse is an optimization-based network embedding method which optimizes an objective function that minimizes the Kullback-Leibler (KL) divergence from the given similarity distribution in graph space to similarity distribution in embedding space. The objective function is given as follows :
\begin{equation}
    \sum_{v\in V} \; \text{KL} ( sim_G(v,.) \| sim_E(v,.))
\end{equation}
The similarity distribution in graph space could be constructed with help of Personalized PageRank, SimRank, or Adjacency matrix. Since the objective function is expensive to compute for large graphs, it is approximated by Noise Constrastive Estimation \cite{gutmann2010noise}. 

\textbf{Comments}: We search for following  hyperparameters: Pagerank damping factor $\alpha$ = [0.7, 0.85, 0.9], Negative samples = [3, 10], Embedding dimension = [64, 128, 256].


\item \textbf{SDNE \cite{wang2016structural}}: 
SDNE is a deep autoencoder based network embedding method which optimizes an objective function that preserves both first and second order proximity among nodes in the embedding space. The objective function of SDNE is given below

\vspace{-1.5em}
\begin{equation}
    \mathcal{L}_{joint} = \alpha \mathcal{L}_{1st} +  \mathcal{L}_{2nd} +  \nu  \mathcal{L}_{reg}
\end{equation}

where $\mathcal{L}_{1st}$ and $\mathcal{L}_{2nd}$ are loss functions to preserve first order and second order proximities respectively, while $\mathcal{L}_{reg}$ is the regularizer term. The authors propose a semi-supervised deep model to minimize the mentioned objective function. The deep model consists of two components: supervised and unsupervised. The supervised component attempts to preserve the first order proximity while the unsupervised component attempts to preserve the second-order proximity by minimizing reconstruction loss of nodes. 

\textbf{Comments}: We search for following  hyperparameters:  $\alpha$ = [1e-05, 0.2],  Penalty coefficient $\beta$ = [5, 10], Embedding dimension = [64, 128, 256].


\item \textbf{GAE \cite{kipf2016variational}}:
GAE is a graph autoencoder based network embedding method which minimizes the reconstruction loss of the adjacency matrix. The reconstruction matrix is generated as $\hat{A} = \sigma (ZZ^T)$ where $Z$ is node embeddings generated with Graph Convolutional Networks (GCN) \cite{kipf2017semi} as $Z = GCN(X,A)$ with $X$ as node features. In the case of unattributed graphs, the node feature matrix is an identity matrix. 

\textbf{Comments}: We search for following  hyperparameters:  Epochs = [50, 100], Embedding dimension = [64, 128, 256].

\item \textbf{Watch Your Step \cite{abu2018watch}}: Watch Your Step (WYS) addresses the sensitivity issue of hyper-parameters in the random walk based embedding methods. WYS solves the sensitivity issue with the attention mechanism on the expected random walk matrix. The attention mechanism guides the random walk to focus on short or long term dependencies pertinent to the input graph. The objective function of WYS is given as
\vspace{-0.5em}
\begin{equation}
\begin{aligned}
\mathop{min}_{L,R,q} \quad & \beta \| q\|^2_2 -  \| E[D;q] \circ \log(\sigma(L*R^T)) \\ & -\mathbbm{1} [A = 0 ] \circ  \log(1- \sigma(L*R^T)) \|_1
\end{aligned}
\end{equation}

where $q$ is attention parameter vector, $L$ and $R$ are node embeddings, $E[D;q] $ is expectation on the random walk matrix.

\textbf{Comments}: We search for following  hyperparameters: Learning rate =  [0.05, 0.1, 0.2, 0.5, 1.0], Number of Hops = 5, Embedding dimension = [64, 128, 256].











\end{enumerate}
